Towards a consistent interpretation of AIOps models

Artificial Intelligence for IT Operations (AIOps) has been adopted in organizations in various tasks, including interpreting models to identify indicators of service failures. To avoid misleading practitioners, AIOps model interpretations should be consistent (i.e., different AIOps models on the same task agree with one another on feature importance). However, many AIOps studies violate established practices in the machine learning community when deriving interpretations, such as interpreting models with suboptimal performance, though the impact of such violations on the interpretation consistency has not been studied. In this paper, we investigate the consistency of AIOps model interpretation along three dimensions: internal consistency, external consistency, and time consistency. We conduct a case study on two AIOps tasks: predicting Google cluster job failures, and Backblaze hard drive failures. We find that the randomness from learners, hyperparameter tuning, and data sampling should be controlled to generate consistent interpretations. AIOps models with AUCs greater than 0.75 yield more consistent interpretation compared to low-performing models. Finally, AIOps models that are constructed with the Sliding Window or Full History approaches have the most consistent interpretation with the trends presented in the entire datasets. Our study provides valuable guidelines for practitioners to derive consistent AIOps model interpretation.

==> 07.1-discussion1.tex <==
\subsection{Which source of randomness contributes the most to the instability of model interpretation?}

In RQ1, we showed that all three sources of randomness that we studied (i.e., ML learner, randomized hyperparameter tuning, and data sampling) introduce instability to the interpretation of AIOps models. When all three sources of randomness are controlled, we observed identical interpretations of AIOps models across iterations, i.e., the interpretation is fully reproducible. To further understand the scale of instability introduced by each studied source of randomness, we here discuss the comparison of the distributions of Kendall's W from Figure~\ref{fig:rq1.1}, Figure~\ref{fig:rq1.2}, Figure~\ref{fig:rq1.3} and Figure~\ref{fig:rq1.4}. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/Discussion_randomness.pdf}
    \caption{The interpretation stability (measured by Kendall's W) of models when different sources of randomness are not controlled. Each subplot has four boxplots, from left to right represents the control group (all sources of randomness controlled), randomness from ML learner, hyperparameter tuning, and data sampling. See Table~\ref{tab:rq1_setup} for detailed setup.}
    \label{fig:discussion_randomness}
\end{figure}

Figure~\ref{fig:discussion_randomness} provides an aggregated view of the distribution of Kendall's W when different sources of randomness are not controlled, in comparison to a controlled group with all sources of randomness controlled. It can be observed from Figure~\ref{fig:discussion_randomness} that generally when randomness from data sampling is introduced, the interpretation of AIOps models show the lowest agreement; followed by hyperparameter tuning which shows the second lowest agreement among model interpretations. The ML learner's inherent randomness appears to introduce the least instability to AIOps model interpretation. Such observation is consistent across most learners and datasets, except for Multi-layer Perceptron Neural Network (NN) - in the case of NN, hyperparameter tuning introduces comparable interpretation instability to data sampling. A possible explanation is that for NN, the architecture of the network (e.g., the size of hidden layers) are tuned as part of hyperparameter, which may result in significant difference in trained models. Because of the wide adoption of Neural-Network-based learners in AIOps research (e.g., Deep Neural Network, DNN), future work is needed to further explore the impact of hyperparameter tuning randomness on DNN model interpretation.

==> 07.2-discussion2.tex <==
\subsection{Can we suggest best-performed \jack{best-performing?} learners in AIOps solutions?}

In RQ2, we apply a learner-agnostic approach to cluster the models based on their performance.
In this section, we revisit the performance of all the models we trained in RQ2 and group the models based on their underlying learners. For each dataset, we group the models trained on the same period of data by the learners. For models built with each learner, we compute how many of these models are in the best-performing cluster.
For example, in Google dataset, we trained 70 models using the 7 learners on the first period of data. To compute the percentage of models trained using RF in the best-performing cluster, we first count the total number of models in the best-performing cluster. Out of 70 models, there are 8 models in the best-performing cluster. Among them, 5 models are trained using RF. Hence, the percentage of RF learner in the best-performing cluster of the first period is 62.5\%.
For each learner, we repeat the process for each period of data, and then compute the percentage. We summarize the overall distribution using boxplot shown in Figure~\ref{fig:discussion_top_learner}. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/Discussion_top_learner.pdf}
    \caption{Percentage of models trained with each learner in the best-performing cluster.}
    \label{fig:discussion_top_learner}
\end{figure}

For the Google dataset, the results show that RF and GBDT perform much better than other learners. The median percentage of RF and GBDT are around 50\% and the percentage of other five learners are all below 1\%. This finding shows that, in all the studied periods of data, the best-performing models are mostly trained using either RF or GBDT.

Similarly, the results on the Backblaze dataset show that RF and GBDT are still the top two learners among all seven learners. Different from the results on the Google dataset, the performance of models trained using LDA, QDA, LR, and NN are comparable to those trained using RF and GBDT. In general, none of the learners achieve more than 25\%. 

The findings suggest that we should consider using RF and GBDT as the preferred learners in the AIOps context, as they consistently perform the best among all studied learners. In addition, the performance of learners may vary due to different characteristics of different datasets. The correlation between the dataset and performance of learners is not fully explored and we plan to investigate further in the future.

==> 20-temp_tables.tex <==



